Powerline Tracking with Event Cameras

Autonomous inspection of powerlines with quadrotors is challenging. Flights require persistent perception to keep a close look at the lines. We propose a method that uses event cameras to robustly track powerlines. Event cameras are inherently robust to motion blur, have low latency, and high dynamic range. Such properties are advantageous for autonomous inspection of powerlines with drones, where fast motions and challenging illumination conditions are ordinary. Our method identifies lines in the stream of events by detecting planes in the spatio-temporal signal, and tracks them through time. The implementation runs onboard and is capable of detecting multiple distinct lines in real time with rates of up to $320$ thousand events per second. The performance is evaluated in real-world flights along a powerline. The tracker is able to persistently track the powerlines, with a mean lifetime of the line $10\times$ longer than existing approaches.

==> imgs/fig_computational_cost_all.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.85\linewidth] {imgs/computational_cost_all_steps.eps}
    
    \caption{Processing time of different steps as a percentage of the overall processing time.}
    \label{fig:processing_time_bar}
\end{figure}

==> imgs/fig_drone.tex <==

\begin{figure}[tbh]
    \centering
    \includegraphics[width=0.95\linewidth] {imgs/hw_test_drone_setup.png}
    
    \caption{The drone setup used for hardware tests.}
    \label{fig:drone_setup}
\end{figure}


==> tables/table_parameters.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|}
\hline
\textbf{Parameter}      & \textbf{Value} & \textbf{Description}                                                                                                                     \\ \hline
\multicolumn{3}{|l|}{\textbf{Lines}}                                                                                                                                                \\ \hline
promotion threshold     & 1.2 pixel            & \begin{tabular}[c]{@{}l@{}} value of smallest eigenvalue for line promotion\end{tabular}                                  \\ \hline
promotion number events & 35             & \begin{tabular}[c]{@{}l@{}}{[}{]} minimum number\\  of events in cluster \\ for line promotion\end{tabular}                              \\ \hline
initialization length   & 70            & \begin{tabular}[c]{@{}l@{}}{[}px{]} minimum length\\  of line to pass \\ initialization\end{tabular}                                     \\ \hline
initialization period   & 90             & \begin{tabular}[c]{@{}l@{}}{[}ms{]} initialization \\ period\end{tabular}                                                                \\ \hline
addition threshold      & 1.8            & \begin{tabular}[c]{@{}l@{}}{[}px{]} max distance \\ to inferred line for\\  event to be added\end{tabular}                               \\ \hline
merge angle             & 8              & \begin{tabular}[c]{@{}l@{}}{[}deg{]} max angle \\ difference between \\ lines to be merged\end{tabular}                                  \\ \hline
merge distance          & 3.5            & \begin{tabular}[c]{@{}l@{}}{[}px{]} max distance \\ of mid point to other\\  line to be merged\end{tabular}                              \\ \hline
hibernation density     & 0.08           & \begin{tabular}[c]{@{}l@{}}{[}events / (px\textasciicircum{}2 * ms){]} \\ min line density before\\  going into hibernation\end{tabular} \\ \hline
cleanup event age       & 50             & \begin{tabular}[c]{@{}l@{}}{[}ms{]} max age of \\ events before they \\ are removed\end{tabular}                                         \\ \hline
deletion no events      & 200            & \begin{tabular}[c]{@{}l@{}}{[}ms{]} if there have not\\  been any events \\ for longer than this, \\ the line is deleted\end{tabular}    \\ \hline
\multicolumn{3}{|l|}{\textbf{Clusters}}                                                                                                                                             \\ \hline
creation number events  & 7              & \begin{tabular}[c]{@{}l@{}}{[}{]} min number of \\ events to create a \\ cluster from a chain\end{tabular}                               \\ \hline
addition threshold      & 1.3            & \begin{tabular}[c]{@{}l@{}}{[}px{]} max distance \\ to inferred line for \\ an event to be added\end{tabular}                            \\ \hline
merge angle             & 15             & \begin{tabular}[c]{@{}l@{}}{[}deg{]} max angle \\ difference between \\ cluster to be merged\end{tabular}                                \\ \hline
cleanup event age       & 50             & \begin{tabular}[c]{@{}l@{}}{[}ms{]} max age of \\ events before they \\ are removed\end{tabular}                                         \\ \hline
deletion no events      & 40             & \begin{tabular}[c]{@{}l@{}}{[}ms{]} if there have \\ not been any events\\ for longer than this, \\ the cluster is deleted\end{tabular}  \\ \hline
\end{tabular}
\end{table}
